simTPM: User-centric TPM for Mobile Devices (Technical Report)

Trusted Platform Modules are valuable building blocks for security solutions and have also been recognized as beneficial for security on mobile platforms, like smartphones and tablets. However, strict space, cost, and power constraints of mobile devices prohibit an implementation as dedicated on-board chip and the incumbent implementations are software TPMs protected by Trusted Execution Environments. In this paper, we present simTPM, an alternative implementation of a mobile TPM based on the SIM card available in mobile platforms. We solve the technical challenge of implementing a TPM2.0 in the resource-constrained SIM card environment and integrate our simTPM into the secure boot chain of the ARM Trusted Firmware on a HiKey960 reference board. Most notably, we address the challenge of how a removable TPM can be bound to the host device's root of trust for measurement. As such, our solution not only provides a mobile TPM that avoids additional hardware while using a dedicated, strongly protected environment, but also offers promising synergies with co-existing TEE-based TPMs. In particular, simTPM offers a user-centric trusted module. Using performance benchmarks, we show that our simTPM has competitive speed with a reported TEE-based TPM and a hardware-based TPM.

==> chapters/DBmeasurements.tex <==
%!TEX root=usenix2019_v2.tex




==> chapters/androidBackground.tex <==
 


==> chapters/answeringShortComing.tex <==
%!TEX root=NDSS_2018bare_final.tex

In this section we will talk about how \ournameplain overcomes the shortcomings of trusted module in mobile devices. We will one by one show how it achieves all the properties that we have identified in Table~\ref{tab:countermeasures}. Later in use-case section we will talk how to implement the features from Table~\ref{table:relatedworkSynopsisFeatures} with \ournameplain along with some other use-cases. 

NV-storage inside the SIM card solves the problem of having a \textit{secure persistence storage} (\textbf{A1 : \tick}). Smart cards allow the conservation of the card and preserving the current content by preventing updates of the internal state from outside world (\textbf{S1 : \tick}). T%his features prevents modification of its memory from outside. 
To update the content in the NV-storage an external entity has to issue a command known to the card and upon proper authorization will update the storage (\textbf{S2 : \tick}) or perform PCR extension to update PCR content. 

The property that is immediately fulfilled by \ournameplain is \textit{Rollback protection}, due to the secure persistent storage of the smart card. System software or any user level application can keep a sealed counter (\textbf{S5 : \tick}) inside the NV-storage containing the current version of the software (\textbf{S3 : \tick}). Any update carrying a version number lower than the stored counter will be rejected.

%\subsection{PCR Bank}

\ournameplain is equipped with a PCR bank of 24 PCRs (automotive \tpm can have more PCRs). Their contents are initialize at boot-cycle. The content cannot be changed but can only be extended using \textit{PCR\_EXTEND}. In our case PCR 1 to PCR 5 contains the measurements for boot-loaders (2, 3-1, 3-2, 3-3) (boot-loader1 is the starting point of the chain of trust and set as trust anchor. No entity is present to measure boot-loader1 ). PCR 6 is kept for TEE and PCR 7-12 for un-trusted operating system measurements. We did not implement any debug PCR but it can be implemented easily. And rest of the PCRs are kept for application or user specific support.

Presence of PCR bank gives the power of attestation and authorization due to the point that a PCR value cannot be undone. A PCR cannot be rolled back to a previous value. 

%\subsection{Memory isolation}

By design a sim-card offers memory isolation by keeping the memory module on a separate chip from the system (\textbf{S7 : \tick}). Modification of this memory is possible only by card applet upon receiving some command from outside world of the card. The module is connected over a separate bus to the main processing unit.

Secure endorsement can be easily achieved for \ournameplain bu putting an endorsement key inside its storage, keeping in mind that the private part of the key is never visible outside of the \tpm (\textbf{S4 : \tick}). If the \tpm is issued by the carrier then the sim card encryption key can be used as endorsement key providing one extra layer of security due to unavailability of the EK inside the TPM applet but shared between sim and \tpm applet.

%\subsection{Process isolation}

The sim card that we have used in \ournameplain architecture is equipped with a 16-bit processor. The processor is not having enough power to perform normal day computation but it is powerful enough to generate an ECC key or encrypt/decrypt/hash a file (\textbf{S7 : \tick}) or execute \tpm related commands. The size of the file does matter as bigger the file longer the computation on file will take place. But the complete computation will take place on the processor on the sim-card not on the main processing unit. So sniffing the processing is impossible.

%\subsection{Cryptography}

Like any other \tpm, \ournameplain is also equipped with a limited cryptographic capability. Due to processing power limitation, performing fancy cryptographic algorithm is not possible. But \ournameplain is equipped with ECC key generation and encryption protocol, SHA256 and SHA1 hashing algorithm and a hardware based random number generator. 

%\subsection{Secure I/O}

%\ournameplain can easily be used to secure peripheral devices (\textbf{P6 : \tick}). For example a full disk encryption an be implemented just by keeping the encryption key inside the isolated persistence storage of \tpm . Enrollment of a device can be done securely by a challenge-response game initiated by \ournameplain with the help of PCR bank, where the measurements related to peripherals are stored in \ournameplain.

%\subsection{Attestation}

%\subsection{Authentication}

Authentication can be achieved by using a privacy CA setup in addition to \ournameplain on mobile device. The privacy CA will carry the list of trusted sim-\tpm . Also it will carry a list of rogue \tpm s. Network communication signed by trusted sim-\tpm will be  granted keeping in mind that the trusted \tpm authenticated the user. If the communication is signed by a bad \tpm, then the communication will be dropped immediately.

%\subsection{Authorization}

%\subsection{Clock availability}

SIM cards are equipped with a clock pin connected to the baseband processor. SIM card gets its clock signal from the baseband processor which cannot be clocked higher or lower by a normal application or un-trusted operating system. This separate clock helps \ournameplain to work on a different clock frequency not under direct influence of the main processor. What is more, the baseband processor can send APDU commands that contain the current time to the smart card independently of the main CPU  (\textbf{S6 : \tick}).

%\subsection{Early availability}

One of the unique features of \ournameplain architecture in comparison to other available trusted module design for mobile domain is its early availability of \tpm on mobile phones (\textbf{A2 : \tick}). Previous smart-card based mtm implementations lags this feature. \ournameplain is available before machine boots up. As a result it can be counted on as a place to store measurements taken during the boot process. The PCR bank implementation is used for this purpose. Generally the sim applet is locked by user pin issued by the mobile carrier. But this can work as expected and can be unlocked later when the OS boots up successfully.

The other unique feature of the architecture is its move-ability  (\textbf{D2 : \tick}). \ournameplain implements the \tpm inside the sim-card. So by design the \tpm can move with the sim card if the user moves it. This creates some interesting use-cases. In section~\ref{sec:usecase:msm} we will discuss in details

\ournameplain can successfully integrate multiple stakeholder model proposed by TCG  (\textbf{A3 : \tick}). In section~\ref{systemDeign:bindingWithDeviceAndUser} \&~\ref{sec:usecase:switchingSIM} we will discuss in details how move-ability of \tpm can be tackled.

%\subsection{Mobile availability}

The main purpose of this project is to make a trusted platform module available for mobile domain. Integrating it inside a sim card helped us to achieve the purpose (\textbf{D1 : \tick}). As we already discussed that our goal will be not introducing a new chip, rather reuse the existing technologies. We have extended the mobile domain with a physical off-chip hardware \tpm without changing the mobile eco-system. 

%Now wee will indicate how we are achieving the features a trusted module on mobile can provide from table~\ref{table:relatedworkSynopsisProperties}.
%
%\subsection{Authenticated boot or Secure boot}

%\begin{figure*}
%	\centering
%	\includegraphics[width=2.0\columnwidth]{figures/quaSIModo_AuthBoot}
%	\caption{}
%	\label{fig:quaSIModo_AuthBoot}
%\end{figure*}

%\subsection{Digital rights management}

%\subsection{Migration possibility}
%
%\begin{itemize}
%	\item Answer Table I
%\end{itemize}  


==> chapters/currentTechs.tex <==
 


==> chapters/futureWorks.tex <==
%!TEX root=NDSS_2018bare_final.tex

\subsection{Trusted HW for mobile}

\subsection{Options for corporate devices}

This probably the best working situation for \ournameplain. If the phone has multiple sim slot and one slot is always empty, then the empty slot can be used for a dedicated \tpm chip for the phone. In this case binding to the device will be easier as the \tpm chip will never leave (still a removable sim card) the phone. For corporate devices where keeping the integrity untouched for devices are very important, this setup can be very useful. The \stpm will be locked using a key managed by the system administrator. Supported by a CA, the system will be even stronger.

\subsection{Trusted HW for IOT}

\ournameplain setup can help to create an trusted infrastructure for \textit{Internet Of Things (iot)} devices. The prescribed setup will implement one \stpm in the phone, in the iot manager device and individual \stpm s in iot devices. All the iot \tpm s will be initialized and attested by the phone's \tpm. All the commands issued to the iot devices will be authenticated using sign and verify. Also some measurements along with the corresponding identity in the iot manager. This infrastructure will bind the iot devices to one mobile device, reducing unauthenticated and vulnerable iot communication protocol~\cite{RonenOSW16}. 

\subsection{TPM for cars}

\tpm for cars is not a new concept. It already exists but all of the existing systems are embedded on chip. But the move-ability of \ournameplain can improve the usability of \tpm.  


==> chapters/overviewSIM.tex <==
%!TEX root=NDSS_2018bare_final.tex

 


==> chapters/securityAnalysis.tex <==
%!TEX root=NDSS_2018bare_final.tex

In this subsection we briefly discuss the security guarantees that \ournameplain provides. In particular, we argue that beside problems arising from the move-ability of \stpm$, it provides the same security guarantees as a hardware \tpm. Similar to the threat model of \tpm we do not consider physical attacks here. 

\subsection{Off-Chip protection}

Similar to a hardware \tpm chip, \ournameplain implements an off-board \tpm on the SIM card. This chip is connected to the CPU via system bus communication. Unlike, present day software implementations, it is not susceptible to software rollback attack (section~\ref{relatedworkARMTZ}) and not prone to flawed implementations of entry functions to the secure world (section~\ref{relatedWork:TEE}). Though it is vulnerable to advance attacks on bus communication~\cite{conf/uss/Kauer07, TPMHWattack}.

\ournameplain provides complete isolation of the trusted memory and processing due to 
tamper-resistance of the smart card and its capability of storing data.
%its capability of carrying a small amount of memory on board and a low power processor. 
In comparison, software \tpm solutions lack in memory and processing isolation and they have to rely RAM memory.
%The isolation also provides security over side channel attacks due to not sharing resources with the untrusted OS.

\subsection{Time based Side-Channel Attacks}

To be compliant with the \tpm 2.0 specification the \tpm has to implement cryptographic functions
that are resilient to timing based side-channel attack. We have a similar requirement for smart card which are designed to be resistant against all types of side-channel attacks. Thus, \ournameplain immediately makes itself resilient to time based side channel attacks.

%\subsection{Other attacks}
%
%Due to design, \ournameplain is easily affected by wrong movement of sim-card from the phone. \vphantom{But this physical access to the mobile device or sim-card which we assume is hard.} An uneducated movement of \ournameplain over different phones can remove all the measurements it is holding for authenticated boot and can jeopardize the phones trust. But a little knowledge on howto can improve the trust on the mobile system greatly.

%\subsection{Secure clock}
%
%We need an implementation of secure clock for two reasons. 1) First use is to measure lockout duration. After entering password for a number of times, \tpm goes for a lockout to prevent dictionary attack or password guessing award. 2) Secondly the clock can be used for a timed authorization. For example a key issued for one hour will become unusable. \ournameplain gets its clock from a separate base-band processor from the board. This prevents the possibilities of vulnerabilities related to over clocking or under clocking. 

